Random Forest Models for Accurate Identification of Coordination Environments from X-ray Absorption Near-Edge Structure

Analyzing coordination environments using X-ray absorption spectroscopy has broad applications ranging from solid-state physics to material chemistry. Here, we show that random forest models can identify the main coordination environment from K-edge X-ray absorption near edge structure (XANES) with a high accuracy of 85.4% and all associated coordination environments with a high Jaccard score of 81.8% for 33 cation elements in oxides, significantly outperforming other machine learning (ML) models. In a departure from prior works, we used a robust description of the coordination environment as a distribution over 25 distinct coordination motifs with coordination numbers ranging from 1-12. The random forest models were trained on the world's largest database of ~190,000 computed K-edge XANES spectra. Furthermore, the random forest models can be applied to predict the coordination environment from experimental K-edge XANES with minimal loss in accuracy (82.1%) due to the use of data augmentation. A drop-out feature importance analysis highlights the key roles that the pre-edge and main-peak regions play in coordination environment identification, with the post-peak region becoming increasingly important at higher coordination numbers. This work provides a general strategy to identify the coordination environment from K-edge XANES across broad chemistries, paving the way for future advancements in the application of ML to spectroscopy.

==> dummy_mkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
